Canonical Fields: Self-Supervised Learning of Pose-Canonicalized Neural Fields

Coordinate-based implicit neural networks, or neural fields, have emerged as useful representations of shape and appearance in 3D computer vision. Despite advances, however, it remains challenging to build neural fields for categories of objects without datasets like ShapeNet that provide "canonicalized" object instances that are consistently aligned for their 3D position and orientation (pose). We present Canonical Field Network (CaFi-Net), a self-supervised method to canonicalize the 3D pose of instances from an object category represented as neural fields, specifically neural radiance fields (NeRFs). CaFi-Net directly learns from continuous and noisy radiance fields using a Siamese network architecture that is designed to extract equivariant field features for category-level canonicalization. During inference, our method takes pre-trained neural radiance fields of novel object instances at arbitrary 3D pose and estimates a canonical field with consistent 3D pose across the entire category. Extensive experiments on a new dataset of 1300 NeRF models across 13 object categories show that our method matches or exceeds the performance of 3D point cloud-based methods.

==> content/tables/ablation_gradient.tex <==
\begin{table}[h]
\centering
\scalebox{0.9}{
\begin{tabular}{c|cc}
% \hline
\toprule
\multicolumn{1}{c|}{{\textbf{Category}}}                          & \multicolumn{2}{c}{\textbf{Density vs. Gradient Signals}}                                  \\ \cmidrule{1-3} 
\multicolumn{1}{c|}{}                                                          & \multicolumn{1}{c}{\textbf{Density}} & \multicolumn{1}{c}{\textbf{Gradient signal}}\\ \midrule
% \hline
% \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{GC (partial)}}}  &
\multicolumn{3}{l}{\textbf{Ground Truth Equivariance Consistency (GEC)}{\color{blue} $\downarrow$}} \\
\midrule
\multicolumn{1}{l|}{\textbf{bench}}            & 2.13                   & \textbf{1.85}                                 \\ %\cline{2-6} 
% \multicolumn{1}{c|}{}                                         & 
\multicolumn{1}{l|}{\textbf{cellphone}}            & \textbf{2.59}                  & 3.53                    \\ %\cline{2-6} 
% \multicolumn{1}{c|}{}                                         & 
\multicolumn{1}{l|}{\textbf{chair}}            & 3.77                  & \textbf{3.13}                   \\ %\cline{2-6}
% \multicolumn{1}{c|}{} &
\multicolumn{1}{l|}{\textbf{plane}}            & \textbf{3.43}                  & 4.24                  \\ \midrule %\cline{2-6} 
% \multicolumn{1}{c|}{}                                         & 
\multicolumn{1}{l|}{Average} & \textbf{2.98}          & 3.19                      \\ \midrule
\multicolumn{3}{l}{\textbf{Instance-Level Consistency (IC)}{\color{blue} $\downarrow$}} \\
\midrule
% \hline
% \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{IC (partial)}}}   &
\multicolumn{1}{l|}{\textbf{bench}}            & 1.76                   & \textbf{1.51}                   \\ %\cline{2-6} 
% \multicolumn{1}{c|}{}                                         & 
\multicolumn{1}{l|}{\textbf{cellphone}}            & \textbf{1.64}                   & 2.4       \\ %\cline{2-6} 
% \multicolumn{1}{c|}{}                                         & 
\multicolumn{1}{l|}{\textbf{chair}}            &\textbf{1.27}                   & 1.82                    \\ %\cline{2-6} 
% \multicolumn{1}{c|}{}                                         & 
\multicolumn{1}{l|}{\textbf{plane}} & \textbf{2.36}          & 2.9                     \\ \midrule
% \multicolumn{1}{c|}{}                                         & 
\multicolumn{1}{l|}{Average} & \textbf{1.76}          & 2.16                      \\ \midrule


\multicolumn{3}{l}{\textbf{Category-Level Consistency (CC)}{\color{blue} $\downarrow$}} \\
\midrule
    %  \hline
% \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{CC (partial)}}} & 
\multicolumn{1}{l|}{\textbf{bench}}            & 2.81                   & \textbf{2.65}            \\ %\cline{2-6} 
% \multicolumn{1}{c|}{}                                         & 
\multicolumn{1}{l|}{\textbf{cellphone}}            & \textbf{2.38}                  & 6.55                   \\ %\cline{2-6} 
% \multicolumn{1}{c|}{}                                         & 
\multicolumn{1}{l|}{\textbf{chair}}            & \textbf{4.95}                  & 7.39                   \\ %\cline{2-6} 
% \multicolumn{1}{c|}{}                                         & 
\multicolumn{1}{l|}{\textbf{plane}} & \textbf{4.1}          & 4.81                   \\ \midrule
% \hline
\multicolumn{1}{l|}{\textbf{Average}}   & \textbf{3.56}                  & 5.34          \\ \midrule
\end{tabular}
}
\caption{\textbf{Siamese Training} - w/o - without, w \label{tab:ablation_grad}} 
\end{table}

==> content/tables/ablation_local_average.tex <==
\begin{table}[h]
\centering
\scalebox{0.9}{
\begin{tabular}{c|cc}
% \hline
\toprule
\multicolumn{1}{c|}{{\textbf{Category}}}                          & \multicolumn{2}{c}{\textbf{Local Average}}                                  \\ \cmidrule{1-3} 
\multicolumn{1}{c|}{}                                                          & \multicolumn{1}{c}{\textbf{Density }} & \multicolumn{1}{c}{\textbf{Gradient signal}}\\ \midrule
% \hline
% \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{GC (partial)}}}  &
\multicolumn{3}{l}{\textbf{Ground Truth Equivariance Consistency (GEC)}{\color{blue} $\downarrow$}} \\
\midrule
\multicolumn{1}{l|}{\textbf{bench}}            & \textbf{2.13}                   & 2.21                                \\ %\cline{2-6} 
% \multicolumn{1}{c|}{}                                         & 
\multicolumn{1}{l|}{\textbf{cellphone}}            & \textbf{2.59}                  & 2.96                   \\ %\cline{2-6} 
% \multicolumn{1}{c|}{}                                         & 
\multicolumn{1}{l|}{\textbf{chair}}            & \textbf{3.77}                  & 5.21                  \\ %\cline{2-6}
% \multicolumn{1}{c|}{} &
\multicolumn{1}{l|}{\textbf{firearm}}            & 1.77                  & \textbf{1.72}                 \\ \midrule %\cline{2-6} 
% \multicolumn{1}{c|}{}                                         & 
\multicolumn{1}{l|}{Average} & \textbf{2.57}          & 3.03                      \\ \midrule
\multicolumn{3}{l}{\textbf{Instance-Level Consistency (IC)}{\color{blue} $\downarrow$}} \\
\midrule
% \hline
% \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{IC (partial)}}}   &
\multicolumn{1}{l|}{\textbf{bench}}            & \textbf{1.76}                   & 1.84                  \\ %\cline{2-6} 
% \multicolumn{1}{c|}{}                                         & 
\multicolumn{1}{l|}{\textbf{cellphone}}            & \textbf{1.64}                   & 2.09       \\ %\cline{2-6} 
% \multicolumn{1}{c|}{}                                         & 
\multicolumn{1}{l|}{\textbf{chair}}            &\textbf{1.27}                   & 4.14                   \\ %\cline{2-6} 
% \multicolumn{1}{c|}{}                                         & 
\multicolumn{1}{l|}{\textbf{firearm}} & \textbf{0.78}          & 0.86                    \\ \midrule
% \multicolumn{1}{c|}{}                                         & 
\multicolumn{1}{l|}{Average} & \textbf{1.36}          & 2.23                      \\ \midrule


\multicolumn{3}{l}{\textbf{Category-Level Consistency (CC)}{\color{blue} $\downarrow$}} \\
\midrule
    %  \hline
% \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{CC (partial)}}} & 
\multicolumn{1}{l|}{\textbf{bench}}            & \textbf{2.81}                   & 2.87            \\ %\cline{2-6} 
% \multicolumn{1}{c|}{}                                         & 
\multicolumn{1}{l|}{\textbf{cellphone}}            & \textbf{2.38}                  & 2.92                  \\ %\cline{2-6} 
% \multicolumn{1}{c|}{}                                         & 
\multicolumn{1}{l|}{\textbf{chair}}            & \textbf{4.95}                  & 7.11                   \\ %\cline{2-6} 
% \multicolumn{1}{c|}{}                                         & 
\multicolumn{1}{l|}{\textbf{firearm}} & 2.93          & \textbf{2.39}                  \\ \midrule
% \hline
\multicolumn{1}{l|}{\textbf{Average}}   & \textbf{3.27}                  & 3.82          \\ \midrule
\end{tabular}
}
\caption{\textbf{Siamese Training} - w/o - without, w \label{tab:ablation_grad}} 
\end{table}

==> content/tables/ablation_siamese.tex <==
\begin{table}[h]
\centering
\scalebox{0.9}{
\begin{tabular}{c|cc}
% \hline
\toprule
\multicolumn{1}{c|}{{\textbf{Category}}}                          & \multicolumn{2}{c}{\textbf{Siamese Training}}                                  \\ \cmidrule{1-3} 
\multicolumn{1}{c|}{}                                                          & \multicolumn{1}{c}{\textbf{w/o siamese}} & \multicolumn{1}{c}{\textbf{with siamese}}\\ \midrule
% \hline
% \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{GC (partial)}}}  &
\multicolumn{3}{l}{\textbf{Ground Truth Equivariance Consistency (GEC)}{\color{blue} $\downarrow$}} \\
\midrule
\multicolumn{1}{l|}{car}            & 2.76                   & \textbf{1.56}                                 \\ %\cline{2-6} 
% \multicolumn{1}{c|}{}                                         & 
\multicolumn{1}{l|}{chair}            & 3.43                   & \textbf{3.77}                   \\ %\cline{2-6} 
% \multicolumn{1}{c|}{} &
\multicolumn{1}{l|}{plane}            & 5.82                  & \textbf{3.43 }                  \\ %\cline{2-6} 
\multicolumn{1}{l|}{bench}            & \textbf{1.95 }                  & 2.13                   \\ \midrule
\multicolumn{1}{l|}{Average} & 3.49          & \textbf{2.72}                     \\ \midrule
\multicolumn{3}{l}{\textbf{Instance-Level Consistency (IC)}{\color{blue} $\downarrow$}} \\
\midrule
% \hline
% \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{IC (partial)}}}   &
\multicolumn{1}{l|}{car}         & 1.87                   & \textbf{1.44}                   \\ %\cline{2-6} 
% \multicolumn{1}{c|}{}                                         & 
\multicolumn{1}{l|}{chair}            & 1.74                  & \textbf{1.27}           \\ %\cline{2-6} 
% \multicolumn{1}{c|}{}                                         & 
\multicolumn{1}{l|}{plane}      & 3.93                   & \textbf{2.36}                    \\ %\cline{2-6} 
% \multicolumn{1}{c|}{}                                         & 
\multicolumn{1}{l|}{bench}           & 2.33                  & \textbf{1.76}                   \\ \midrule %\cline{2-6} 
\multicolumn{1}{l|}{Average} & 2.96          & \textbf{1.71}                  \\ \midrule
\multicolumn{3}{l}{\textbf{Category-Level Consistency (CC)}{\color{blue} $\downarrow$}} \\
\midrule
    %  \hline
% \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{CC (partial)}}} & 
\multicolumn{1}{l|}{car}            & 3.19                   & \textbf{1.96}            \\ %\cline{2-6} 
% \multicolumn{1}{c|}{}                                         & 
\multicolumn{1}{l|}{chair}            & 7.54                   & \textbf{4.95}                 \\ %\cline{2-6} 
% \multicolumn{1}{c|}{}                                         & 
\multicolumn{1}{l|}{plane}            & 6.23                  &\textbf{4.1}                 \\ %\cline{2-6} 
% \multicolumn{1}{c|}{}                                         & 
\multicolumn{1}{l|}{bench}            & 2.64                  & 2.81                           \\ \midrule
% \hline
\multicolumn{1}{l|}{\textbf{Average}}   & 4.9                  & \textbf{3.21}          \\ \midrule
\end{tabular}
}
\caption{\textbf{Siamese Training} - w/o - without, w \label{tab:ablation_siamese}} 
\end{table}

==> content/tables/pcd.tex <==
\begin{table}[h]
\centering
{
\scalebox{0.7}{
\begin{tabular}{c|cc}
% \hline
\toprule
% \multicolumn{1}{c|}{{\textbf{Category}}}                          & \multicolumn{2}{c}{\textbf{Shapenet surface Point clouds vs. Nerf extracted point clouds}}                                  \\ \cmidrule{1-3} 
\multicolumn{1}{c|}{\textbf{Category}} & \multicolumn{1}{c}{\textbf{ShapeNet}} & \multicolumn{1}{c}{\textbf{NeRF pointclouds}}\\ \midrule
% \hline
% \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{GC (partial)}}}  &
\multicolumn{3}{l}{\textbf{Ground Truth Equivariance Consistency (GEC)}{\color{blue} $\downarrow$}} \\
\midrule
\multicolumn{1}{l|}{\textbf{Chair}}       & 0.85     & 3.98         \\ 
\multicolumn{1}{l|}{\textbf{Table}}     & 1.2     & 3.45         \\ 
\multicolumn{1}{l|}{\textbf{Car}}         & 0.61     & 0.17         \\ 
\midrule %
        


\multicolumn{3}{l}{\textbf{Instance-Level Consistency (IC)}{\color{blue} $\downarrow$}} \\
\midrule


\multicolumn{1}{l|}{\textbf{Chair}}       & 0.21     & 1.53         \\ 
\multicolumn{1}{l|}{\textbf{Table}}     & 0.47     & 1.72         \\ 
\multicolumn{1}{l|}{\textbf{Car}}     & 0.12   & 0.37         \\ 
\midrule 


\multicolumn{3}{l}{\textbf{Category-Level Consistency (CC)}{\color{blue} $\downarrow$}} \\
\midrule
\multicolumn{1}{l|}{\textbf{Chair}}       & 0.77     & 2.86         \\ 
\multicolumn{1}{l|}{\textbf{Table}}     & 1.14     & 3.73         \\ 
\multicolumn{1}{l|}{\textbf{Car}}     & 0.52   & 2.77         \\ 
\midrule %
\end{tabular}
}}
\vspace{-0.3cm}
\caption{Ablation studies}
\label{tab:ablation}
\end{table}
\vspace{-0.1cm}

==> content/text/04_method_backup.tex <==
\input{content/Figures/pipeline}
%
\section{Method}
% \Rahul{Change according to current expt}
\label{sec:method}
%
Given a pre-trained implicit radiance field $f_{r}: \mathbb{R}^3 \to (\textbf{c}, \sigma)$ of a single-object scene, our method estimates a canonicalizing transformation that aligns objects to a category-level consistent frame of reference. Estimating this pose-invariant canonical embeddings that represent a shape enables tasks such as classification, part segmentation and more. Working directly over implicit fields enables \ShortName to canonicalize in-the-wild captured implicit reconstructions. Our work does not assume pre-canonicalized dataset and estimates a pose-invariant canonical frame in an un-supervised manner. We borrow ideas from \cite{sajnani2022condor} and extend them to canonicalize noisy in-the-wild density fields from NeRF reconstructions.
\Rahul{I have created a backup of this file and changing in the new file}

\subsection{Sampling and Preprocessing}

We begin by sampling a density field to obtain the reconstruction of the object of interest. The sampled densities are then canonicalized for scale, translation, and rotation. \ShortName predicts a pose-invariant canonicalizing coordinate for each point in the density field and estimates a canonicalizing transform that aligns the grid to a category-level canonical frame. The predicted canonical coordinates are transformed to the input coordinate frame to penalize for self-supervised consistency that canonicalize shapes without any supervision (\ref{} \Rahul{Add pipeline figure}).

\todo{In particular, we use the density field from NeRF and discard the direction-dependent color.}



\parahead{Preprocessing} We hierarchically sample the pre-trained NeRF model wherein the first sampling step finds the extremities of the object and the object center by weighing queried locations by their respective normalized density. The second sampling step uniformly samples the object within the extremities at $\epsilon$ interval around the center of the object $\textbf{c}$ and scales it to unit dimensions.  
% \Rahul{Random perturbation?}
% \Rahul{@Rohith please mention the details of how you sample}. 
We obtain a uniformly sampled density grid $\bm{\sigma}_D \in \mathbb{R}^{H \times W \times D}$ by querying the density radiance model $f_r^{\sigma}$ along with their sampling locations $\bm{X} \in \mathbb{R}^{H \times W \times D \times 3}$.% and color $\bm{C}_D \in \mathbb{R}^{H \times W \times D \times 3}$. 
\begin{align*}
    &\bm{X} = \{x \;|\; x \in [\textbf{c}-l/2 : \epsilon : \textbf{c}+l/2] \} \\
    &\bm{\sigma}_D = \{1 - exp(-d \cdot f^{\sigma}_r(x)) \;|\; x \in \bm{X}\}
\end{align*}
Here, $l$ is the maximal diagonal length of the object and $d$ is a hyper-parameter that is constant across all scenes. The query locations are with respect to the scene that is not consistent with the canonical frame.  Note that the density processed by $(1 - exp(\cdot))$ lies in the continuous range $[0, 1]$. 

\todo{We tried both grid and random density sampling, grid worked just as well.}

% \Rahul{Centering field such that object is at origin}
\subsection{Robust Equivariant Features}
We use spherical harmonic functions to build equivariant learnable features and use equivariant non-linearities from \cite{poulenard2021functional} to construct our architecture. 

\parahead{Input feature types} \ShortName uses density $\bm{\sigma}_D$ as a type 0 feature and compute its discrete gradient ($\nabla \bm{\sigma}_D \in \mathbb{R}^{H \times W \times D \times 3}$) wherein $\nabla \bm{\sigma}_D = \{(f^{\sigma}_r(x + \Delta x) - f^{\sigma}_r(x - \Delta x))/(2\Delta x)\; | \; x \in \textbf{X}\}$ for very small $\Delta x$ and sets it as a type-1 equivariant feature that is input to our network. Gradients are type-1 equivariant signals that capture small irregularities within the object to improve canonicalization (see ablation \cref{sec:expt}). 
% \Rahul{Cross-check and change accordingly}


% \parahead{Equivariant Convolution} Each layer in \ShortName employs equivariant convolution with equivariant non-linearities \cite{poulenard2021functional} that mixes type-$n$ steerable kernels $k^{n}_r(\cdot)$ with type-$\ell$ signals $s^{\ell}$ and decompose it to irreducible features of different types using Clebsh-Gordon decomposition \cite{thomas2018tensor}. The Equivariant Convolution (EConv) at location ${}^{R}x$ is as follows:
% \begin{align*}
%     & \text{EConv}^{J}({}^Rx) = Q^{(n,\ell), J}\left(\sum_{{}^{R/2}y \in \mathcal{N}} k^{n}_r({}^{R}x - {}^{R/2}y) \otimes s^{\ell}[{}^{R}x]\right)%\\
%     %& W^{J} \text{EQConv}^{J}({}^Rx) + \delta_{J0}b
% \end{align*}
% Here, $R$ is the sampling resolution wherein we sample the implicit field at resolutions $\frac{1}{2}, \frac{1}{4}$, and $\frac{1}{8}$. ${}^{R/2}y$ is the neighbor of ${}^{R}x$ at half the resolution and $\otimes$ is the tensor product operation. Instead of using the type-1 $xyz$ grid locations, we use the gradient as type-$1$ feature at every resolution of our architecture to perform our convolution.

% This convolution  The kernel at a particular resolution uses the difference of 3D points at the grid location $X_D$ with their respective nearest neighbors from grid locations sampled at half the resolution to capture global equivariant features. 


% We compute the steerable kernels for a point location x as follows:
% \begin{align*}
%     k^{n}_r(x - y) = \{\varphi_r(\norm{x - y}_2) Y^{n}\left(\frac{x - y}{\norm{x - y}_2}\right)
% \end{align*}

% Where $\varphi_r$ is the normalizing function defined in \cite{poulenard2021functional} and $y$ are nearest neighbors of $x$ that are sampled at half the resolution. 



\parahead{Weighing features by density}
The density sampled from NeRF reconstructions are often noisy and contain outliers. To guide the learning to learn from locations with higher density, we weigh each equivariant feature type by a function of its density. Features from the first layer are weighed by their local averaged density to smoothen the signal and avoid small noisy patches that do not correspond to the object. These equivariant features are weighed by their corresponding point densities for the remaining layers as the receptive field of the convolution increases. We learn equivariant features of type $J$ with weights $W^{J}$ and $b$ as follows:

\begin{align*}
    & {}^{R}s^{\ell} =  f_{w}({}^{R}x) \left(W^J (\text{EQConv}^J({}^{R}x)) + \delta_{0J}b\right) \\
    &f_{w}({}^{R}x)=
    \begin{cases}
      \text{mean}_{r} (\bm{\sigma}_D({}^{R}x)), & \text{if}\ R = 1/2 \\
      \bm{\sigma}_D({}^{R}x), & \text{otherwise}
    \end{cases}
\end{align*}
Here, ${}^{R}x$ is a 3D point queried at resolution $R$ and $\text{mean}_{r} (\bm{\sigma}_D({}^{R}x))$ is the average density at point $^{R}x$ from points sampled at radius $r$. We aggregate features at resolutions $\frac{1}{2}, \frac{1}{4}$, and $\frac{1}{8}$. The $\text{EQConv}^{J}$ layer is as defined in \cref{sec:background}.
We employ non-linearities from \cite{poulenard2021functional} and compute max-pool of point-wise features of the last layer to obtain global type-$\ell$ equivariant features $F^{\ell}$. RGB features from the network are not used to process

\todo{Why RGB is not used? Perhaps because of view-dependence?}

\subsection{Implicit field Canonicalization }

After obtaining the global type-$\ell$ equivariant feature $F^{\ell}$, we compute its dot product with point-wise Spherical Harmonics $Z^{\ell}$ scaled by their norms $Z^{\ell}(\bm{X}) = \norm{\bm{X}}_2 Y^{\ell}(\bm{X}/\norm{\bm{X}}_2)$ to obtain a pose-invariant embedding $H^{\ell}$ \cite{sajnani2022condor}. As the two vectors $F^{\ell}$ and $Z^{\ell}$ are both equivariant to input rotation, their dot products are invariant. We linear layer on top of the pose-invariant embedding to estimate point coordinates in the canonical frame ($Y \in \mathbb{R}^{H \times W \times D \times 3}$) for each point in $\bm{X}$ and $M$ equivariant transformations $E \in \mathbb{R}^{M \times 3 \times 3}$ \cite{sajnani2022condor} that orient the canonical coordinates to the input coordinates. We then choose the best canonicalizing transform $E_{b}$ and penalize for canonicalization. This is done as below:
\begin{align*}
    & H^{\ell}(\bm{X}) = \langle F^{\ell}, Z^{\ell}(\bm{X}) \rangle \\
    & Y = \text{MLP}_{Y}(H(\bm{X})) \\
    & E = \text{MLP}_{E}(F(\bm{X}))
\end{align*}
Here, we have dropped the type-$\ell$ notation for $H$ and $F$ as we concatenate all type features. 

%According to our experiments (\ref{}), weighing equivariant features by locally averaged density and then canonicalizing rejects outliers for small patches to improve canonicalization. 


\subsection{Training}
\ShortName predict a canonical coordinate for every point in space, but unlike point clouds, fields have many un-occupied regions that do not provide any information. We penalize the network on foreground regions only by performing K-means clustering on the densities with $K = 2$ and choose the cluster $\bm{C}_f$ with higher mean. Note that we operate on continuous fields, but only cluster to weigh loss functions that guide our training.
% \Rahul{@Rohith How do we know which cluster is fg? Is it the one with the higher mean?}. 

\subsubsection{Loss functions}

\parahead{Canonicalization loss} To self-supervise our learning, we transform the predicted canonical coordinates to the input coordinates and compute a point-wise L2-distance between the input coordinates and the canonical coordinates transformed to the input by the best transformation $E_b$.

\begin{align*}
    & E_b = \min_{j} (\text{mean}_{i \in \bm{C}_f} \norm{\bm{X}_i - E_j Y_i}_2^{2})\\
    & \mathcal{L}_{canon} = \text{mean}_{i \in \bm{C}_f} \norm{\bm{X}_i - E_b Y_i}_2^2
\end{align*}

\parahead{Orthonormality loss} The predicted equivariant transformations should have orthonormal vectors and we use the following to force orthonormality:
\begin{align*}
    & U_j, D_j, V_j = \text{SVD}(E_j)\\
    & \mathcal{L}_{ortho} = \text{mean}_j \norm{E_j - U_j V^{T}_j}_2
\end{align*}

$\text{SVD}(E_j)$ computes the singular value decomposition of the $j^{th}$ equivariant transformation.

% \parahead{Inter-object consistency}
\subsubsection{Architecture and hyper-parameters}

\subsubsection{Dual branch arch? helpful or not}



% \Rahul{
% \begin{enumerate}
%     \item Change in kernel and incorporating density
%         \begin{itemize}
%             \item Instead of using the regular Euclidean distance to select the neighbourhood we modified the selection criteria to Euclidean distance / Density (This really not helped that much very slight improvement)  
%         \end{itemize}
%     \item Incorporating gradient signals and various types + what all helped
%             \begin{itemize}
%                 \item we tried experiments with multiple equivariant signals derived from density and sample locations includes density (type 0) , gradient of the density (type 1) , CB Decomposition of Hessian of Density field and Tensor product between the points and Gradient fields . out of all gradients seems working good.
%                 \item as the gradients are sensitive to noise we wanted to weight each point feature by some confidence score which should be equivaraint. one choice would be using  the point density as weighing factor.  second one would be taking the local avg densities of the neighbourhood points. second choice improved the performance over the first choice.   
%             \end{itemize}
%     \item Clustering
%           \begin{itemize}
%               \item 
%           \end{itemize}
%     \item Loss functions
% \end{enumerate}}

==> content/text/rebuttal/00_rebuttal.tex <==
% \noindent % Don't mess with the review template
We thank the reviewers for their valuable feedback and positive comments about our work such as ``the paper addresses an important problem and is one of the first to do so directly with NeRF'' (\Rone, \Rthree) and has the ``potential to have a significant impact on the field of 3D computer vision'' (\Rtwo). Reviewers agree that our method ``makes sense and the results are promising" (\Rthree) and that ``the proposed scheme extends the concept of feature equivariance to NeRFs" (\Rone). They also comment that we ``thoroughly evaluate the proposed method" (\Rtwo) to canonicalize NeRFs by creating and using ``a large scale [1300 trained NeRFs] dataset for the problem'' (\Rthree).
We share the reviewers' positive outlook of the paper, and address any remaining concerns and factual errors below.
% We address the reviewers' concerns and detail ways to improve the paper below.
% "created a dataset to train and thoroughly evaluate the proposed method" (R2, R3), "extends the concept of feature equivariance...to NeRFs" (R1). All reviewers agree that it is a "Well-written paper". 

\parahead{Sampling Bounding Box vs.~Frustum (\Rone)}
%
We are not fully sure what \Rone{} means by using frustum sampling as opposed to uniform sampling for canonicalizing fields.
In the following, we assume that \Rone's suggestion is to sample points within the intersection/union of all camera frustums of a NeRF scene. Sampling the intersection of all camera frustums can lead to missing the object within the scene if one of the views does not capture it. On the other hand, sampling the union of camera frustums becomes too complex as the number of cameras increase. 
%\Rahul{} 
The reason we chose uniform grid sampling was because we \textbf{do not} assume any knowledge about \textbf{camera extrinsics} during inference -- we consider only the trained NeRF model (without the original images) as the input.
This makes our method more general and allows it to operate on a NeRF model with unknown camera extrinsics and original images. 
% Sampling the intersection of camera frustums results in missing the object if not present in one of the views. 
% \Rahul{We do need scene bounds though, should I mention or ignore? Ignore}.
% Furthermore, a scene may have cameras that do not contain the object at all in the camera frustum.
% In this setting, sampling points at the intersection of all camera frustums would miss sampling regions of the object that aren't in the intersection and result in improper canonicalization.


\parahead{Justification of Failure Cases (\Rone)}
%
Our method fails to canonicalize a few instances that have poor NeRF reconstructions or thin/symmetric shapes, for instance, a few NeRF models of chairs have very thin legs and aren't reconstructed properly making it difficult to canonicalize them.
As theoretically shown in \cite{balachandar2022breaking}, the components in the direction of symmetry are zero for equivariant neural networks.
This creates an ambiguity when estimating the canonical frame, resulting in a few shapes that do not align with the other instances of the category.
We will include this theoretically-motivated justification in the final manuscript.
% explain and justify this in more detail in the main paper.
% We observed that our method failed for a few instances and understood this to be due to the relatively poor quality of fields and/or the lack of sufficient occupancy in the fields corresponding to these instances.

\parahead{Perceived Underperformance in some Cases (\Rone)}
%
Our ConDor (P) comparison operates on pointclouds extracted from NeRF whereas our method operates directly on densities with uncertain occupancy values.
Canonicalizing densities with uncertainty is more difficult as the uncertainty increases for very thin/small structures that could be missed.
Furthermore, densities contain occupied as well as unoccupied regions.
Our method needs to attend and learn equivariant features from the foreground region of the field which is significantly harder.
Even so, our method performs comparably in most cases (Table~1, main paper).
% SOTA pointcloud canonicalizer ConDor, and \textbf{does not} underperform
We will include this justification in the final manuscript.
% We justify this based on the fact that our method works with probabilistic inputs such as densities, which inherently have uncertainty and noise.
% This results in poorer performance compared to methods that operate directly on pointclouds where occupied regions are known with certainty.
% However, it is worth noting that our method is on par with the best-performing methods even for such categories.
% \srinath{Contradiction: how can we be on-par if results are poorer? This para needs improvement.}

\parahead{Comparison with ``Clean'' Surface Pointcloud Methods
% Without Using NeRF as Intermediate Step 
(\Rthree)}
%
\Rthree{} suggested that it may be useful to compare the canonicalization performance of prior methods (e.g.,~ConDor) operating on clean \emph{surface-only} pointclouds extracted from ShapeNet meshes.
We agree this could be useful, but also want to point out that this is not the paper's goal -- we want to demonstrate that canonicalization is possible directly from noisy NeRF reconstructions rather than clean surface pointclouds.
% Furthermore, ShapeNet pointclouds have points only on the surface and do not have inherent noise that is present in NeRF reconstructions.
% Our work primarily focuses on displaying that canonicalization is possible with implicit density fields.
% Nonetheless, we conducted a minor experiment and report results for three categories \{\textit{car, airplane, chair}\}in \cref{tab:ablation}. 
Nonetheless, we conducted a minor experiment as requested.
We trained ConDor on clean ShapeNet surface pointclouds and obtained metrics: (\textbf{GEC:} $\mathbf{0.90}$, \textbf{IC:} $\mathbf{0.31}$, \textbf{CC:} $\mathbf{0.87}$) on average over all categories.
For ConDor trained on NeRF-extracted pointclouds, we obtained: (\textbf{GEC:} $\mathbf{3.04}$, \textbf{IC:} $\mathbf{1.65}$, \textbf{CC:} $\mathbf{2.90}$).
%
The difference between these two different settings is expected because ShapeNet pointclouds do not have noise and contain points only on the object surface.
However, NeRF-extracted pointclouds are noisy, and contain more number of points because we capture both the surface and the interior -- thus, this is not a fair comparison.
% which is not the setting of our work.
% $GEC$ of $0.89$ and report the mean and median of canonicalizing ShapeNet pointclouds and NeRF extracted pointclouds. 
% All the metrics (\textit{IC, CC, GEC}) are higher for NeRF extracted pointclouds as compared to ShapeNet pointclouds on average for all the categories. ShapeNet  
% All the metrics are inferior for NeRF pointclouds as opposed to ShapeNet pointclouds (apart from GEC metric for car) as NeRF pointclouds have points within the surface as well as contain noise.   
% \srinath{What does the table show? Anaylze the results.}
% Comparing canonicalization performance on \shaurya{grammatically incomplete} without extracting pointclouds from NeRF is not exactly apples to apples as the representations are different.
% Even though CVPR guidelines discourage new experiments, we present a minor additional experiment displaying metrics obtained from ConDor without intermediate NeRF reconstruction as \Rthree{} requested.
%
% \input{content/tables/pcd}
% In Table 1, we present the metric values obtained from the other methods with this change.

\parahead{Reference (\Rtwo{})}
%
We thank \Rtwo{} for referring us to \cite{seo2022equisym} and will explore ways to incorporate the ideas from this work to address the symmetry problem in the future.

\parahead{Other Comments (\Rone{}, \Rtwo{}, \Rthree{})}
We thank the reviewers for all the other comments and suggestions on typos, grammar, and writing -— we will address them in final version of the manuscript. 

To summarize, we address the problem of canonicalizing NeRFs in a self-supervised setting and create a large dataset of 1300 NeRF models to evaluate it.
During inference our method canonicalizes a NeRF model of a novel object instance from the same category.
% Our canonicalization results in estimating pose invariant features that can be leveraged for future applications. 
Furthermore, reviewers' commented that our is the ``first solution to directly canonicalize a novel unseen NeRF of a new object instance in a self-supervised scheme", is an ``important contribution" (\Rone{}), and can ``potentially be useful for NERF-based recognition".
% are more positive than their respective scores.
We hope that we have addressed all the questions and concerns raised by reviewers \Rone{} and \Rthree{}, and hope that they will consider increasing their scores.
% the concerns addressed in this rebuttal.

% \srinath{End with a positive statement (quote from reviewers) and encourage the WA reveiwers to raise their score. Something like ``we hope that R1 and R3 with consider increasing their score.} 

==> content/text/rebuttal/10_template.tex <==
%%%%%%%%% BODY TEXT - ENTER YOUR RESPONSE BELOW
\section{Introduction}

After receiving paper reviews, authors may optionally submit a rebuttal to address the reviewers' comments, which will be limited to a {\bf one page} PDF file.
Please follow the steps and style guidelines outlined below for submitting your author response.

The author rebuttal is optional and, following similar guidelines to previous CVPR conferences, is meant to provide you with an opportunity to rebut factual errors or to supply additional information requested by the reviewers.
It is NOT intended to add new contributions (theorems, algorithms, experiments) that were absent in the original submission and NOT specifically requested by the reviewers.
You may optionally add a figure, graph, or proof to your rebuttal to better illustrate your answer to the reviewers' comments.

Per a passed 2018 PAMI-TC motion, reviewers should refrain from requesting significant additional experiments for the rebuttal or penalize for lack of additional experiments.
Authors should refrain from including new experimental results in the rebuttal, especially when not specifically requested to do so by the reviewers.
Authors may include figures with illustrations or comparison tables of results reported in the submission/supplemental material or in other papers.

Just like the original submission, the rebuttal must maintain anonymity and cannot include external links that reveal the author identity or circumvent the length restriction.
The rebuttal must comply with this template (the use of sections is not required, though it is recommended to structure the rebuttal for ease of reading).

%-------------------------------------------------------------------------

\subsection{Response length}
Author responses must be no longer than 1 page in length including any references and figures.
Overlength responses will simply not be reviewed.
This includes responses where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.

%------------------------------------------------------------------------
\section{Formatting your Response}

{\bf Make sure to update the paper title and paper ID in the appropriate place in the tex file.}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The top margin should begin 1 inch (2.54 cm) from the top edge of the page.
The bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the page.

Please number any displayed equations.
It is important for readers to be able to refer to any particular equation.

Wherever Times is specified, Times Roman may also be used.
Main text should be in 10-point Times, single-spaced.
Section headings should be in 10 or 12 point Times.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Figure and table captions should be 9-point Roman type as in \cref{fig:onecol}.


List and number all bibliographical references in 9-point Times, single-spaced,
at the end of your response.
When referenced in the text, enclose the citation number in square brackets, for example~\cite{Alpher05}.
Where appropriate, include the name(s) of editors of referenced books.

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{0.5in} \rule{0.9\linewidth}{0pt}}
  %\includegraphics[width=0.8\linewidth]{egfigure.eps}
   \caption{Example of caption.  It is set in Roman so that mathematics
   (always set in Roman: $B \sin A = A \sin B$) may be included without an
   ugly clash.}
   \label{fig:onecol}
\end{figure}

To avoid ambiguities, it is best if the numbering for equations, figures, tables, and references in the author response does not overlap with that in the main paper (the reviewer may wonder if you talk about \cref{fig:onecol} in the author response or in the paper).
See \LaTeX\ template for a workaround.

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
Please ensure that any point you wish to make is resolvable in a printed copy of the response.
Resize fonts in figures to match the font in the body text, and choose line widths which render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your response in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it is almost always best to use \verb+\includegraphics+, and to specify the  figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}

